Stable and Transferable Hyper-Graph Neural Networks

We introduce an architecture for processing signals supported on hypergraphs via graph neural networks (GNNs), which we call a Hyper-graph Expansion Neural Network (HENN), and provide the first bounds on the stability and transferability error of a hypergraph signal processing model. To do so, we provide a framework for bounding the stability and transferability error of GNNs across arbitrary graphs via spectral similarity. By bounding the difference between two graph shift operators (GSOs) in the positive semi-definite sense via their eigenvalue spectrum, we show that this error depends only on the properties of the GNN and the magnitude of spectral similarity of the GSOs. Moreover, we show that existing transferability results that assume the graphs are small perturbations of one another, or that the graphs are random and drawn from the same distribution or sampled from the same graphon can be recovered using our approach. Thus, both GNNs and our HENNs (trained using normalized Laplacians as graph shift operators) will be increasingly stable and transferable as the graphs become larger. Experimental results illustrate the importance of considering multiple graph representations in HENN, and show its superior performance when transferability is desired.

==> scratch.tex <==
\begin{enumerate}
    \item Introduce GNNs, hypergraphs, robustness via transferability/stability
    \item Spectral similarity and its practicality: given any two graphs, can measure similarity
    \item Compare notions of transferability for GNNs: small perturbations, graphs from same latent space, graphs from same graphon
    \item Transferability/stability via spectral similarity
    \item Spectral similarity of perturbations
    \item HGNNs (and first trans./stab. result)
    \item Experiments with HGNNs vs GNNs
    \item Experiments with perturbations?
\end{enumerate}






\begin{table*}[t]
    \centering
    \caption{Types of Hypergraph Shift Operators}
    
    \begin{tabular}{|c|c|}
        \hline
        Architecture & Hypergraph convolutional layer \\
        \hline
        Clique-Line (Ours) & $\begin{aligned}
            X_v^{l+1} &= \sigma\left(\sum_{k=0}^K (D_v^{-1/2}BWB^\intercal D_v^{-1/2})^k X_v^l H_k^l\right) \\
            X_e^{l+1} &= \sigma\left(D_{ee}^{-1/2}B^\intercal BW D_{ee}^{-1/2}X_e^l H_k^l\right)
            \end{aligned}$ \\
        HGNN \cite{feng2019hypergraph} & $X^{l+1} = \sigma\left(D_v^{-1/2}BWD_e^{-1}B^\intercal D_v^{-1/2}X^l H\right)$ \\
        HGNN+ \cite{gao2022hgnn} & $X^{l+1} = \sigma\left(D_v^{-1}BWD_e^{-1}B^\intercal X^l H\right)$ \\
        HyperAtten \cite{bai2021hypergraph} & $X^{l+1} = \sigma\left(D_v^{-1/2}\tilde{B}WD_e^{-1}\tilde{B}^\intercal D_v^{-1/2} X^l H\right)$ \\
        HyperGCN \cite{yadati2019hypergcn} & $X^{l+1} = \sigma\left(\tilde{D}_v^{-1/2}\tilde{B}WD_e^{-1}\tilde{B}^\intercal \tilde{D}_v^{-1/2} X^l H\right)$ \\
        HNHN \cite{dong2020hnhn} & $\begin{aligned}
            X_e &= \sigma(D_e^{-1}B^\intercal D_v X^l H_v^l) \\
            X^{l+1} &= \sigma(D_v^{-1} B D_e X_e H_e^l)
        \end{aligned}$ \\
         \hline
    \end{tabular}
\end{table*}

\subsection{Transferability of spectrally similar graphs}

Consider two undirected graphs $\cG$ and $\tilde{\cG}$ with shift operators $S = V\Lambda V^\intercal$ and $\tS = \tV \tLambda \tV^\intercal$, respectively. Assume they are spectrally similar, i.e., there is some small $\epsilon$ such that $(1-\epsilon)\lambda_i \leq \tlambda_i \leq (1+\epsilon)\lambda_i$ for all $i = 1,\ldots,n$. Our problem is stated below.

\HR{I'm surprised our problem statement has nothing to do with hypergraphs...}

{\color{red}This entire intro section still needs rewriting, ignore it for now}

\begin{problem}
Given a GNN trained on $\cG$ using $S$, can we bound the difference between its output and the output of the same GNN using $\tS$, the shift operator for $\tilde{\cG}$? In particular, for some arbitrary node signal $x$, can we bound the quantity
\begin{align}
\normed{\Phi(\cdot; S,\cH) - \Phi(\cdot; \tS,\cH)}.
\end{align}
\end{problem}



In particular,
\begin{align*}
    ||y - \ty||_2 &= \Bigg|\Bigg|\sum_{k=0}^\infty h_k(S^k - \tS^k)x\Bigg|\Bigg|_2 \\
        &\leq \sum_{k=0}^\infty ||h_k(S^k - \tS^k)x||_2 \\
        &\leq \sum_{k=0}^\infty h_k||S^k - \tS^k||_F||x||_2 \\
        &= \sum_{k=0}^\infty h_k||V\Lambda^kV^\intercal - \tV\tLambda^k\tV^\intercal||_F||x||_2. %\\
        %&= \sum_{k=0}^\infty h_k||(V - \tV)(\Lambda^k - \tLambda^k)(V^\intercal - \tV^\intercal) - V(\Lambda^k - \tLambda^k)\tV^\intercal - \tV(\Lambda^k - \tLambda^k)V^\intercal - \tV\Lambda^k\tV^\intercal - V\tLambda V^\intercal||_F||x||_2
\end{align*}
By spectral similarity, we know that
\begin{align*}
    &(1-\epsilon)|\lambda_i| \leq |\tlambda_i| \leq (1+\epsilon)|\lambda_i| \\
    \Rightarrow~& (1-\epsilon)^k|\lambda_i|^k \leq |\tlambda_i|^k \leq (1+\epsilon)^k|\lambda_i|^k \\
    \Rightarrow~&  (|\tlambda_i|^k - |\lambda_i|^k)^2 \leq ((1+\epsilon)^k - 1)^2|\lambda_i|^{2k}.
\end{align*}
If the graph shift operators are Laplacian matrices, the absolute values are not necessary. Moreover, Davis-Kahan theorem allows us to obtain bounds on quantities such as $||V - \tV||_F$, although in practice we use a projection matrix onto some subset of the eigenvectors. Can we put these things together to obtain a transferability bound? For example,
\begin{align*}
    ||(V - \tV)(\Lambda^k - \tLambda^k)(V^\intercal - \tV^\intercal)||_F &\leq ||V - \tV||_F^2||\Lambda^k - \tLambda^k||_F \\
    &= ||V - \tV||_F^2\cdot\text{trace}((\Lambda^k - \tLambda^k)^\intercal(\Lambda^k - \tLambda^k))^{1/2} \\
    &= ||V - \tV||_F^2\left(\sum_{i=0}^n(\lambda_i^{k} - \tlambda_i^k)^2\right)^{1/2} \\
    &\leq ||V - \tV||_F^2\left(\sum_{i=0}^n((1+\epsilon)^k - 1)^2\lambda_i^{2k}\right)^{1/2} \\
    &= ((1+\epsilon)^k - 1)||V - \tV||_F^2||\Lambda^{2k}||_F
\end{align*}
where the first normed quantity can be bounded by Davis-Kahan, and the overall bound will be small if $k$ and $\epsilon$ are small. If the GSO is the Laplacian matrix, then we also have that $||\Lambda^{2k}||_F \leq n(2d_{max})^{2k}$, where $d_{max}$ is the largest degree of any node in $\cG$. However, in practice this will be a loose bound.




Convergence and stability of GNNs on large random graphs \cite{keriven2020convergence}, universality of GNNs on large random graphs  \cite{keriven2021universality}, convergence of generalized Erdos-Renyi graphs \cite{chakrabarty2021spectra} (related but not necessarily the semicircle law).

\subsection{Stability for random graphs}

Results of \cite{tao2012topics}, specifically showing small perturbations result in the same limiting distribution.

We present a result from \cite{tao2012topics} which illustrates that empirical spectral distributions are stable with respect to low-rank and small-magnitude perturbations. In particular, via \Cref{thm:Wigner_TF_bound}, GNNs trained on appropriate GSOs of random graphs are stable with respect to such perturbations. Combining this result with those from \Cref{sec:random_transferability}, we see that the normalized Laplacian of large graphs drawn from many common random graph families will produce trained GNNs that are both stable and transferable across the family.


\begin{theorem}[Stability of empirical spectral distributions \cite{tao2012topics}]
Let $\{S_n\}_{n=1}^\infty$ be a sequence of real symmetric random matrices such that $\mu_{n^{-1/2}S_n} \to \mu$ in probability. Furthermore, let $\{D_n\}_{n=1}^\infty$ and $\{E_n\}_{n=1}^\infty$ be sequences of real symmetric random matrices such that $n^{-2}\normed{D_n}_F^2 \to 0$ and $n^{-1}\text{rank}(E_n) \to 0$ in probability. Then $\mu_{n^{-1/2}(S_n + D_n)} \to \mu$ and $\mu_{n^{-1/2}(S_n + E_n)} \to \mu$ in probability.
\end{theorem}

\iffalse\begin{definition}[Wigner matrices]
Given some independent random variables $y_{ij}$, $i\in\{1,\ldots,n\}$, $j\in\{i,\ldots,n\}$, define the symmetric matrix $Y_n \in \R^{n\times n}$ such that
\begin{align*}
    [Y_n]_{ij} = \begin{cases}
        y_{ij}/\sqrt{n}, & i \leq j, \\
        y_{ji}/\sqrt{n}, & i > j.
    \end{cases}
\end{align*}
If the $y_{ij}$ are independent and have finite second moments ($\E[y_{ij}^2] < \infty$), the diagonal entries $\{y_{ii}\}_{i\geq 1}$ are identically distributed, and the off-diagonal entries $\{y_{ij}\}_{1\leq i < j}$ are identically distributed with positive second moments (otherwise $Y_n$ will be diagonal almost surely), then the $Y_n$ are \emph{Wigner matrices}.
\end{definition}\fi

\iffalse
\begin{proposition}[Wigner's semicircle law \cite{erdHos2012rigidity,tao2012topics}]\label{thm:Wigner_law}
For a symmetric matrix $S_n = n^{-1/2}[s_{ij}]_{i,j=1}^n \in\R^{n\times n}$, where $s_{ij}=s_{ji}$ for $j>i$ are independent, identically distributed random variables such that $\E[s_{ij}]=0$ and $\Var[s_{ij}] = 1$, assume the following:
\begin{enumerate}[label=(\emph{A\arabic*})]
    \item $\lambda_1(S_n) = 1$ is a simple eigenvalue of $S_n$ and there is some $c_b > 0$, indepedent of $n$, such that $\{\lambda_i(S_n)\}_{i=1}^n \subset(-1+c_b,1-c_b)\cup\{1\}$;
    \item the distributions of the $s_{ij}$ have a uniformly subexponential decay, i.e., there exists $c_d>0$ such that $P(|s_{ij}| > zn^{-1/2}) \leq e^{-z^{c_d}}/c_d$ for all $z \geq 1$.
\end{enumerate}
Let $\{S_n\}_{n=1}^\infty$ satisfy assumptions \ref{ass:concentration}-\ref{ass:zero_multiplicity}. Then $\mu_{S_n} \to \mu$ in probability as $n \to \infty$. Moreover, given $\epsilon > 0$ and $\delta > 0$, there exists some $N$ large enough  such that for any $n \geq N$, 
\begin{align}\label{eq:rigidity_thm}
    P\left(|\lambda_i(S_n) - \gamma_i| < \epsilon ~\forall i\in\{1,\ldots,n\}\right) > 1 - \delta.
\end{align}
\iffalse
for $N$ large enough, there exist some constants $A_0 > 1$, $C > 0$, $c > 0$, and $0 < \phi < 1$ such that for any $L$ with $A_0\log\log n \leq L \leq \log(10n)/10\log\log n$,
\begin{align}\label{eq:rigidity_theorem}
    &P\left(\ |\lambda_i - \gamma_i| < (\log n)^L\min\{i, n - i + 1\}^{-1/3}n^{-2/3}~\forall i\right) \geq 1 - Ce^{-c(\log n)^{\phi L}}
\end{align}
\fi
\end{proposition}

\begin{remark}
The assumption that $s_{ij}$ have zero-mean and unit variance can easily be relaxed (see, e.g., \cite{chakrabarty2021spectra}). Intuitively, due to the spectral mapping theorem, if $\E[s_{ii}] = \tau$ and $\Var(s_{ij}) = t$ then $\mu_{(t^{-1/2}S_n - \tau)} \to \mu$ in probability as $n \to \infty$ \cite{tao2012topics}. Moreover, the $s_{ij}$ need not be identically distributed  \cite{erdHos2012rigidity}, and it can be shown that these quantities converge almost surely \cite{tao2012topics}.
\end{remark}
\fi

\iffalse
\begin{proposition}[Normalized Laplacian of random graphs \cite{chung2004spectra}]\label{prop:chung_spectra}
Let $\{S_n\}_{n=1}^\infty$ be a sequence of normalized Laplacians of random graphs, where the expected degrees of the nodes of $S_n$ are given by some fixed $w_1,\ldots,w_n$. Define $ w_{min} \coloneqq \min \{w_1,\ldots,w_n\}$ and $w_{avg} \coloneqq 1/n\sum_{i=1}^n w_i$. If $w_{min} \gg \sqrt{w_{avg}}\log^3(n)$, then $\max_i|\lambda_i(S_n)| \approx  2/\sqrt{w_{avg}}$. Moreover, if $w_{min} \gg \sqrt{w_{avg}}$, then $\mu_{1-(4/w_{avg})^{-1/2} S_n} \to \mu$ in probability as $n \to \infty$.
\end{proposition}
\fi

%Of particular interest are \emph{Wigner matrices} $Y_n = [y_{ij}/\sqrt{n}]_{i,j=1}^n$ where the $y_{ii}$ and the $y_{ij}, j > i$ are each independent and identically distributed. Here $\E[y_{ij}^2] = t/n$
\iffalse
\begin{theorem}\label{thm:Wigner_similarity}
Let $\{S_n\}_{n=1}^\infty$ and $\{\tS_n\}_{n=1}^\infty$ be independent sequences of symmetric matrices with i.i.d. entries satisfying the conditions of \Cref{thm:Wigner_law}, such that for some $\tau$ and $t > 0$ we have $\mu_{(t^{-1/2}S_n-\tau)} \to \mu$ and $\mu_{(t^{-1/2}\tS_n-\tau)} \to \mu$ in probability as $n \to \infty$. Assume further:
\begin{enumerate}[label=(\emph{A\arabic*})]
    \setcounter{enumi}{2}
    \item the eigenvalue $0$ has the same multiplicity for $S_n$ and $\tS_n$ (potentially zero);
    \item there exists $c > 0$ such that for any $n$, $|\lambda_i(S_n)| > c$ and $|\lambda_i(\tS_n)| > c$ for all non-zero eigenvalues.
\end{enumerate}
Then for any $\epsilon > 0$ and $\delta > 0$, there exists some large enough $N = N(\epsilon, \delta, t)$ such that for any $n \geq N$,
\begin{align}\label{eq:rigidity}
    P\!\left((1\!-\!\epsilon)\lambda_i < \tlambda_i < (1\!+\! \epsilon)\lambda_i ~\forall i\in\{1,\ldots,n\}\!\right) \!>\! 1 - \delta.
\end{align}
In other words, for matrices of the same size drawn from independent sequences of matrices whose empirical spectral distributions converge to the same semicircle law, the coefficient of spectral similarity converges in probability to $0$ as $n\to\infty$.
\end{theorem}
\fi




\subsection{Nerve complexes}

As discussed earlier, the clique expansion is simply the $1$-skeleton of the simplicial complex, and the line graph of a hypergraph $\cH$ is the $1$-skeleton of the associated nerve complex. Thus, to generalize the notions in the previous section, we now explore how to diffuse these hypergraph node signals across a simplicial complex.

\begin{enumerate}
    \item Construct the nerve complex $\cS$ of the hypergraph $\cH$. The nodes of $\cS$ are the hyperedges of $\cH$, and we construct simplices in $\cS$ between nodes of $\cS$ if the corresponding hyperedges in $\cH$ have nonempty intersection.
    \item Construct signals on the simplices of $\cS$ by pooling node signals of $\cH$. For example, for a simplex $s = \{e_1, e_2, e_3\}$ with $e_1 \cap e_2 \cap e_3 = \{u_1,\ldots,u_k\}$, we would assign a signal to $s$ by pooling the node signals of $u_1,\ldots,u_k$ (e.g., take a maximum or mean).
    \item Construct a HGNN, using the Hodge Lpalacians as shift operators. Depending on the application, signals may be pooled appropriately afterwards.
\end{enumerate}



\color{red}{
\Cref{lem:filter_op_bound} gives us $\normed{H^{fg}_l(S)}_{op} \leq (h_l^{fg}(|\lambda_{max}(S)|))^2 \coloneqq c_l^{fg}$. Thus, notice similarly to \eqref{eq:pf_GNN_output_bound} that
\begin{align*}
    \normed{\bx_{l}^f}_2 &\leq \sum_{g=1}^{f_{l-1}}\normed{H^{fg}_l(S)\bx_{l-1}^g}_2 \\
    &\leq \sum_{g=1}^{f_{l-1}}\normed{H^{fg}_l(S)}_{op} \normed{\bx_{l-1}^g}_2 \\
    &\leq \sum_{g=1}^{f_{l-1}}c_l^{fg} \normed{\bx_{l-1}^g}_2 \\
    &\leq \sum_{g_{l-1}=1}^{f_{l-1}}c_l^{fg_{l-1}} \sum_{g_{l-2}=1}^{f_{l-2}}c_{l-1}^{g_{l-1}g_{l-2}}\cdots\sum_{g_{0}=1}^{f_{0}}c_{1}^{g_{1}g_{0}} \normed{\bx_{0}^{g_{0}}}_2 \\
    &\coloneqq \kappa_l^f,
\end{align*}
where $\bx_o^g$ are the input features. Note the recursive relation $\kappa_l^f = \sum_{g_{l-1}=1}^{f_{l-1}}c_l^{fg_{l-1}}\kappa_{l-1}^{g_{l-1}}$. We stress that $\kappa_l^f$ is a function of the layer, number of features, and the magnitude of the input feature vectors, but also of the largest-magnitude eigenvalue of $S$ via $c_l^{fg}$. Recall that via \Cref{prop:spectral_similarity_bound}, $\normed{H^{fg}_l(S) - H^{fg}_l(\tS)}_{op} \leq C\epsilon + \cO(\epsilon^2)$. Combining these results and applying them recursively,
\begin{align*}
    &\normed{\bx_l^f - \tbx_l^f}_2 \\
    &\leq \cO(\epsilon^2) + f_{l-1}\kappa_{l-1}^f C\epsilon + \sum_{g=1}^{f_{l-1}} c_l^{fg}\normed{\bx_{l-1}^g - \tbx_{l-1}^g}_2 \\
    %%
    &\leq \cO(\epsilon^2) + C\epsilon\Bigg[f_{l-1}\kappa_{l-1}^f + \!\sum_{g_{l-1}=1}^{f_{l-1}}\! c_l^{fg_{l-1}}\!\Bigg(f_{l-2}\kappa_{l-2}^{g_{l-1}} \\
    &\qquad\qquad\qquad\qquad+ \frac{1}{C\epsilon}\!\sum_{g_{l-2}=1}^{f_{l-2}}\! c_{l-1}^{g_{l-1}g_{l-2}}\normed{\bx_{l-2}^{g_{l-2}} - \tbx_{l-2}^{g_{l-2}}}_2\Bigg)\Bigg] \\
    %%
    &\leq \cO(\epsilon^2) + C\epsilon\Bigg[\sum_{g_{l-1}=1}^{f_{l-1}}\! c_l^{fg_{l-1}}\!\Bigg((f_{l-1} + f_{l-2})\kappa_{l-2}^{g_{l-1}} \\
    &\qquad\qquad\qquad\qquad + \sum_{g_{l-2}=1}^{f_{l-2}}\! c_{l-1}^{g_{l-1}g_{l-2}}\normed{\bx_{l-2}^{g_{l-2}} - \tbx_{l-2}^{g_{l-2}}}_2\Bigg)\Bigg] \\
    %%
    &\leq \cO(\epsilon^2) + C\epsilon\Bigg[f_{l-1}\kappa_{l-1}^f + \!\sum_{g_{l-1}=1}^{f_{l-1}}\! c_l^{fg_{l-1}}\!\Bigg(f_{l-2}\kappa_{l-2}^{g_{l-1}}  + \cdots\\
    &\qquad\qquad\qquad + \sum_{g_{1}=1}^{f_{1}}\! c_2^{g_{2}g_{1}}\Bigg(f_1\kappa_1^{g_2} +\!\sum_{g_{0}=1}^{f_{0}}\! c_1^{g_{1}g_{0}}\!\normed{\bx_{0}^{g_{0}} - \tbx_{0}^{g_{0}}}_2\!\Bigg)\!\cdots\!\Bigg]\!.
\end{align*}
Note that the input signals are the same, so $\bx_0^g = \tbx_0^g$ for all $g$. Moreover, if the input signals have unit norm and $|h(\lambda)| \leq c$ then $c_l^{fg}\leq c$ for all $l$, $f$, $g$ and $\kappa_l^f = \kappa_l \leq c^{l-1}\prod_{s=0}^{l-1} f_{s}$. Hence, in this case,
\begin{align*}
    &\normed{\bx_l^f - \tbx_l^f}_2 \\
    &\leq \cO(\epsilon^2) + C\epsilon\Bigg[f_{l-1}\kappa_{l-1} + c f_{l-1} \!\Bigg(f_{l-2}\kappa_{l-2}  + \cdots\\
    &\qquad\qquad\qquad\qquad (f_1\kappa_1 + c f_1 (f_0\kappa_0))\cdots\Bigg] \\
    &= \cO(\epsilon^2) + C\epsilon\sum_{s=1}^l \kappa_{s-1}c^{l-s}\prod_{t=s-1}^{l-1}f_t \\
    &\leq \cO(\epsilon^2) + C\epsilon\sum_{s=1}^l c^{l-s}\prod_{t=s-1}^{l-1}f_t \times c^{s-1}\prod_{\tau=0}^{s-2}f_\tau \\
    &= C\epsilon \left(l c^{l-1} \prod_{t=0}^{l-1} f_t\right) + \cO(\epsilon^2).
\end{align*}
The output signals of the GNNs are the quantities $\{\bx_L^f\}_{f=1}^{f_L}$ and $\{\tbx_L^f\}_{f=1}^{f_L}$. Hence, since we wish to bound the difference in the output of the GNNs, for an arbitrary input signal $\bx_0 = \{\bx_0^f\}_{f=1}^{f_0}$, we have
\begin{align*}
    &\normed{\Phi(\bx_0 ; S,\Theta) - \Phi(\bx_0 ; \tS,\Theta)}_2^2 \\
    &= \sum_{f=0}^{f_L} \normed{\bx_L^f - \tbx_L^f}_2^2 \\
    &\leq C\epsilon \left(L c^{L-1} \prod_{t=0}^{L} f_t\right) + \cO(\epsilon^2)
\end{align*}
Finally, note that if the filter coefficients are normalized so $|h(\lambda)| \leq 1$ (hence $c\leq 1$) and the number of filters at each layer is fixed at $f$, then
\begin{align*}
    \normed{\Phi(\bx_0 ; S,\Theta) - \Phi(\bx_0 ; \tS,\Theta)}_2^2 \leq C L f^L \epsilon + \cO(\epsilon^2).
\end{align*}
and the result is proven.}


\begin{lemma}\label{lem:filter_op_bound}
For a graph filter $H(S)$, we have that 
\begin{align}
    \normed{H(S)}_{op} \leq h(|\lambda_{max}(S)|)^2,
\end{align}
where $\lambda_{max}(S)$ is the largest-magnitude eigenvalue of $S$.
\end{lemma}
\begin{proof}
Let us write $\bx = \sum_{i=1}^n \tx_i \bv_i$ as the graph Fourier representation of $\bx$. Since graph filters are linear operators,
\begin{align*}
    \normed{H(S)}_{op} &= \max_{\normed{\bx}_2=1}\normed{H(S)\bx}_{2} \\
    % &= \max_{\normed{\bx}_2=1}\normed{\sum_{k=0}^K h_{k}S^k\bx}_{2} \\
    &= \max_{\sum_{i=1}^n\tx_i=1}\normed{\sum_{k=0}^K h_{k}S^k\sum_{i=1}^n \tx_i \bv_i}_{2} \\
    &= \max_{\sum_{i=1}^n\tx_i=1}\normed{\sum_{i=1}^n \tx_i\sum_{k=0}^K h_{k} \lambda_i^k\bv_i}_{2} \\
    &= \max_{\sum_{i=1}^n\tx_i=1}\sum_{i=1}^n(\tx_i)^2 \left(\sum_{k=0}^K h_{k} \lambda_i^k\right)^2 \normed{\bv_i}_{2} \\
    &\leq \left(\sum_{k=0}^K h_{k} |\lambda_{max}|^k\right)^2 \\
    &= h(|\lambda_{max}|)^2,
\end{align*}
as desired.
\end{proof}



\iffalse
{\color{red}
Let $\{Y_n\}$ be a sequence of Wigner matrices, with $\E[y_{ij}^2] = t$. We wish to show that Wigner matrices become arbitrarily spectrally similar as they grow larger with high probability. Hence, we will show that for any small $\epsilon \in (0,2]$ and $\delta \in (0,1]$, there exists some $N$ large enough that when independently sampling two Wigner matrices $S,\tS\sim Y_n$,
\begin{align}
    &P\left((1 - \epsilon)\lambda_i(S) \leq \lambda_i(\tS) \leq (1 + \epsilon)\lambda_i(S)~\forall i\right) > 1-\delta \nonumber \\
    \Leftrightarrow~& P\left(|\lambda_i(S) - \lambda_i(\tS)| < \epsilon|\lambda_i(S)|~\forall i\right) > 1-\delta,
\end{align}
for all $n > N$. For large enough $N$, let us fix some $n > N$ and denote $\lambda_i \coloneqq \lambda_i(S)$ and $\tlambda_i \coloneqq \lambda_i(\tS)$.
Let $\gamma_i$, $i\in\{1,\ldots,n\}$, denote the almost surely constant \emph{nominal location} of the $i$-th eigenvalue of a Wigner matrix, i.e., the value $\gamma_i$ such that $\int_{-t}^{\gamma_i} \sigma_t(x)dx=i/n$ (see \cite{erdHos2012rigidity} for details). The eigenvalue rigidity of Wigner matrices $\{Y_n\}$ \cite{erdHos2012rigidity} says that, as $n\to\infty$, the eigenvalues of $Y_n$ concentrate around the values $\gamma_i$. More precisely, for any $\epsilon > 0$ and $\kappa > 0$, we will choose $N$ large enough that $\forall n > N$,
\begin{align}\label{eq:rigidity_assumption}
    &P\left(|\lambda_i(Y_n) - \gamma_i| < \epsilon^2/2\right) > 1 - \kappa \\
    \Rightarrow &P\left(|\lambda_i - \gamma_i| < \epsilon^2/2\right) > 1 - \kappa, \nonumber \\
    &P\left(|\tlambda_i - \gamma_i| < \epsilon^2/2\right) > 1 - \kappa. \nonumber
\end{align}
Here we choose $\kappa = 1 - (1-\delta)^{1/2}$ so that $(1-\kappa)^2 = 1 - \delta$. Moreover, since $P(A) > P(B)$ if $A \supseteq B$ and $\epsilon^2/2 \leq \epsilon$ for $\epsilon \in (0,2]$,
\begin{align}\label{eq:rigidity_pf_bound}
    P\left(|\lambda_i| < |\gamma_i| + \epsilon ~\forall i\right) &\geq P\left(\left||\lambda_i| - |\gamma_i|\right| < \epsilon ~\forall i\right) \nonumber \\
        &\geq P\left(|\lambda_i - \gamma_i| < \epsilon ~\forall i\right) \nonumber \\
        &\geq P\left(|\lambda_i - \gamma_i| < \epsilon^2/2 ~\forall i\right) \nonumber \\
        &> 1 - \kappa.
\end{align}
Denote $\cI \coloneqq \{i\in\{1\ldots,n\} \ | \ |\gamma_i| \geq 2\epsilon\}$ and $\cI^c$ as its complement. Hence, for $N$ large enough we have
\begin{align*}
    &P\left(|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|~\forall i\right) \\
    &= P\left(\cap_{i\in\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\}\cap_{i\in\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\} \right) \\
    &\geq P\Big(\cap_{i\in\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\}\cap\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
        &\quad\qquad\cap_{i\in\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\}\cap\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big),
\end{align*}
by law of total probability. Since $\epsilon^2/2 \leq \epsilon$ for $\epsilon \in (0,2]$,
\begin{align}\label{eq:rigidity_pf_result}
    P(\cap_{i\in\cI}\left\{|\gamma_i| - \epsilon < |\lambda_i|\right\}) &\geq P(\cap_{i\in\cI}\left\{||\lambda_i| - |\gamma_i|| < \epsilon\right\}) \nonumber \\
        &\geq P(\cap_{i\in\cI}\left\{|\lambda_i - \gamma_i| < \epsilon\right\}) \nonumber \\
        &\geq P(|\lambda_i - \gamma_i| < \epsilon^2/2 ~\forall i) \nonumber \\
        &> 1 - \kappa,
\end{align}
and similarly $P(\cap_{i\in\cI^c}\left\{|\lambda_i| < |\gamma_i| + \epsilon\right\}) > 1 - \kappa$. Thus, we are including high-probability events above.
Then, since $|\gamma_i| \leq 2\epsilon$ for $i\in\cI$ and by the triangle inequality, we have
\begin{align*}
    &P\Big(\cap_{i\in\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\}\cap\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
        &\quad\quad\cap_{i\in\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\}\cap\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \\
    &\geq P\Big(\cap_{i\in\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon(|\gamma_i|-\epsilon)\right\}\cap\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
        &{\color{red}\quad\qquad\cap_{i\in\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon(|\gamma_i| + \epsilon)\right\}\cap\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big)} \\
    &\geq P\Big(\cap_{i\in\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon(2\epsilon-\epsilon)\right\}\cap\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
        &\quad\qquad\cap_{i\in\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon(0 + \epsilon)\right\}\cap\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \\
    &= P\Big(\cap_{i=1}^n\left\{|\lambda_i - \tlambda_i| < \epsilon^2\right\}\cap_{i\in\cI}\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
        &\quad\qquad\cap_{i\in\cI^c}\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \\    
    &\geq P\Big(\cap_{i=1}^n\left\{|\lambda_i - \gamma_i| + |\tlambda_i - \gamma_i| < \epsilon^2\right\}\cap_{i\in\cI}\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
        &\quad\qquad\cap_{i\in\cI^c}\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \\
    &\geq P\Big(\cap_{i=1}^n\left\{|\lambda_i - \gamma_i| < \epsilon^2/2\right\}\cap\left\{|\tlambda_i - \gamma_i| < \epsilon^2/2\right\} \\
        &\quad\qquad\cap_{i\in\cI}\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \cap_{i\in\cI^c}\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big).
\end{align*}
Now, by \eqref{eq:rigidity_assumption} and independence of $S$ and $\tS$,
\begin{align*}
    &P\Big(\cap_{i=1}^n\left\{|\lambda_i - \gamma_i| < \epsilon^2/2\right\}\cap\left\{|\tlambda_i - \gamma_i| < \epsilon^2/2\right\} \\
        &\quad\qquad\cap_{i\in\cI}\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \cap_{i\in\cI^c}\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \\
    &= P\Big(\cap_{i=1}^n\left\{|\lambda_i - \gamma_i| < \epsilon^2/2\right\}\cap_{i\in\cI}\left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
        &\quad\qquad \cap_{i\in\cI^c}\left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \times P\left(|\tlambda_i - \gamma_i| < \epsilon^2/2~\forall i\right) \\
    &> (1-\kappa)P\Big(\cap_{i=1}^n\left\{|\lambda_i - \gamma_i| < \epsilon^2/2\right\} \cap \left\{ |\gamma_i| - \epsilon < |\lambda_i|\right\} \\
       &\qquad\qquad\qquad \cap \left\{ |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \\
    %&= (1-\kappa) P\Big(\cap_{i=1}^n\left\{|\lambda_i - \gamma_i| < \epsilon^2/2\right\} \\
    %    &\qquad\qquad\qquad\cap\left\{ |\gamma_i| - \epsilon < |\lambda_i| < |\gamma_i| + \epsilon\right\}\Big) \\
    &= (1-\kappa) P\left(\cap_{i=1}^n\left\{|\lambda_i - \gamma_i| < \epsilon^2/2\right\} \cap\left\{\left||\lambda_i| - |\gamma_i|\right| < \epsilon\right\}\right) \\
    &= (1-\kappa) P\left(|\lambda_i - \gamma_i| < \epsilon^2/2~\forall i\right) \\
    &= (1-\kappa)^2 = 1 - \delta,
\end{align*}
where the third-to-last equality follows from \eqref{eq:rigidity_pf_result}.}
\fi
\iffalse
{\color{red}SCRATCH WORK:
\begin{align*}
    &P\left(|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|~\forall i\right) \\
    &= P\left(|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| ~\forall i \ \Big| \ |\gamma_i| - \epsilon < |\lambda_i| ~\forall i\right) \\
    &\quad\times P\left(|\gamma_i| - \epsilon < |\lambda_i| ~\forall i\right) \\
    &\quad+ P\left(|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| ~\forall i \ \Big| \ \exists i : |\gamma_i| - \epsilon \geq |\lambda_i|\right) \\
    &\quad\times P\left(\exists i : |\gamma_i| - \epsilon \geq |\lambda_i|\right) \\
    &> (1-\kappa)P\left(|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| ~\forall i \ \Big| \ |\gamma_i| - \epsilon < |\lambda_i| ~\forall i\right) \\
    &= (1-\kappa)P\left(\cap_{i\in\cI}\Big\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \ \Big| \ |\gamma_i| - \epsilon < |\lambda_i| \right\} \\
    &\qquad\qquad\qquad\cap_{i\in\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \right\}\Big) \\
    &> (1-\kappa)P\Big(\cap_{\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon(|\gamma_i| - \epsilon) \right\} \\
    &\qquad\qquad\qquad\cap_{\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \right\}\Big) \\
    &> (1-\kappa)P\Big(\cap_{\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon^2 \right\} \\
    &\qquad\qquad\qquad\cap_{\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \right\}\Big) \\
    &= P\left(\cap_{\cI^c}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \right\} \ \Big| \ \cap_{\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \right\}\right) \\
    &\quad\times P\left(\cap_{\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \right\}\right).
\end{align*}
Then by the triangle inequality as well as independence of $S$ and $\tS$ we have
\begin{align*}
    &P\left(\cap_{\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \right\}\right) \\
    &= P\left(\cap_{\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i| \ \Big| \ |\gamma_i| - \epsilon < |\lambda_i| ~\forall i\right\}\right) \\ &\quad\times P\left(\cap_{\cI}\left\{|\gamma_i| - \epsilon < |\lambda_i| \right\}\right) \\
    &> P\left(\cap_{\cI}\left\{|\lambda_i - \tlambda_i| < \epsilon^2 \right\}\right) \\
    &> P\left(|\lambda_i - \tlambda_i| < \epsilon^2 ~\forall i\right) \\
    &=P\left(|\lambda_i - \gamma_i - (\tlambda_i - \gamma_i)| < \epsilon^2 ~\forall i\right) \\
    &> P\left(|\lambda_i - \gamma_i| + |\tlambda_i - \gamma_i| < \epsilon^2 ~\forall i\right) \\
    &> P\left(|\lambda_i - \gamma_i| < \epsilon^2/2 ~\forall i\right)P\left(|\tlambda_i - \gamma_i| < \epsilon^2/2 ~\forall i\right) \\
    &> (1-\kappa)^2.
\end{align*}
Then,
\begin{align*}
    &> (1-\kappa)P\left(|\lambda_i - \tlambda_i| < \epsilon(|\gamma_i|-\epsilon) ~\forall i\right) \\
    &= (1-\kappa)P\left(|\lambda_i - \gamma_i - (\tlambda_i - \gamma_i)| < \epsilon(|\gamma_i|-\epsilon) ~\forall i\right) \\
    &> (1-\kappa)P\left(|\lambda_i - \gamma_i| + |\tlambda_i - \gamma_i| < \epsilon(|\gamma_i|-\epsilon)~\forall i\right) \\
    &> (1-\kappa)P\left(|\lambda_i - \gamma_i| < \epsilon(|\gamma_i|-\epsilon)/2~\forall i\right) \\
    &\quad\times P\left(|\tlambda_i - \gamma_i| < \epsilon(|\gamma_i|-\epsilon)/2~\forall i\right) \\
    &> (1-\kappa)(1-\kappa)^2 \\
    &= 1-\delta.
\end{align*}
where the third- and second-to-last lines hold via eigenvalue rigidity since $S_n$ and $\tS_n$ were independently sampled from the same Wigner matrix distribution. Thus, matrices drawn independently from a Wigner matrix distribution of the same size are $\epsilon$-spectrally similar, where $\epsilon\to 0$ in probability as $n\to\infty$. 
\begin{align*}
    &P\left(|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|~\forall i\right) \\
    &= P\left(\cap_{i=1}^n\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\}\right) \\
    &> P\left(\cap_{|\lambda_i| \geq \epsilon}\left\{|\lambda_i - \tlambda_i| < \epsilon^2\right\} \cap_{|\lambda_i| < \epsilon}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\}\right) \\
    &= P\left(\cap_{|\lambda_i| < \epsilon}\left\{|\lambda_i - \tlambda_i| < \epsilon|\lambda_i|\right\} \ \Big| \ \cap_{|\lambda_i| \geq \epsilon}\left\{|\lambda_i - \tlambda_i| < \epsilon^2\right\}\right) \\
    &~\times P\left(\cap_{|\lambda_i| \geq \epsilon}\left\{|\lambda_i - \tlambda_i| < \epsilon^2\right\}\right)
    % &> (1-\kappa)P\left(\cap_{|\lambda_i| < \epsilon}\left\{|\lambda_i - \tlambda_i| < |\lambda_i|^2\right\} \ \Big| \ \cap_{|\lambda_i| \geq \epsilon}\left\{|\lambda_i - \tlambda_i| < \epsilon^2\right\}\right)
\end{align*}
Moreover, since $P(|\gamma_i| - \epsilon < |\lambda_i| ~\forall i) > 1 - \kappa$, then
\begin{align*}
    1-\kappa &< P\left(|\gamma_i| - \epsilon < |\lambda_i| ~\forall i\right) \\
    &= P\left(\cap_{i=1}^n\left\{|\gamma_i| - \epsilon < |\lambda_i|\right\}\right) \\
    &< P\left(\cap_{|\lambda_i| < \epsilon}\left\{|\gamma_i| - \epsilon < |\lambda_i|\right\}\right) \\
    &< P\left(\cap_{|\lambda_i| < \epsilon}\left\{|\gamma_i| < 2\epsilon\right\}\right)
\end{align*}}
\fi
